Fully-Connected Spatial-Temporal Graph for Multivariate Time-Series Data

Multivariate Time-Series (MTS) data is crucial in various application fields. With its sequential and multi-source (multiple sensors) properties, MTS data inherently exhibits Spatial-Temporal (ST) dependencies, involving temporal correlations between timestamps and spatial correlations between sensors in each timestamp. To effectively leverage this information, Graph Neural Network-based methods (GNNs) have been widely adopted. However, existing approaches separately capture spatial dependency and temporal dependency and fail to capture the correlations between Different sEnsors at Different Timestamps (DEDT). Overlooking such correlations hinders the comprehensive modelling of ST dependencies within MTS data, thus restricting existing GNNs from learning effective representations. To address this limitation, we propose a novel method called Fully-Connected Spatial-Temporal Graph Neural Network (FC-STGNN), including two key components namely FC graph construction and FC graph convolution. For graph construction, we design a decay graph to connect sensors across all timestamps based on their temporal distances, enabling us to fully model the ST dependencies by considering the correlations between DEDT. Further, we devise FC graph convolution with a moving-pooling GNN layer to effectively capture the ST dependencies for learning effective representations. Extensive experiments show the effectiveness of FC-STGNN on multiple MTS datasets compared to SOTA methods. The code is available at https://github.com/Frank-Wang-oss/FCSTGNN.

==> archive/draft.tex <==





\section{related work}


% For example, Zheng et al. \cite{zhang2020tapnet} leveraged CNN to extract features from MTS data, which are used for designed attentional proptotype network to learn features.
% Wang et al. \cite{WANG2019107} proposed multiple CNNs to process the periodic information to make predictions based on MTS data.
% Zheng et al. \cite{zhang2020tapnet} leveraged CNN to extract features from MTS data, which are used for designed attentional proptotype network to learn features. Eldele et al. \cite{eldele2021time} trained a CNN-based encoder with self-supervised paradigm by using unlabeled data only to extract representations from MTS data. 
% For example, Du et al. \cite{DU2020269} proposed a bi-directional-LSTM based model to learn effective representations for MTS forecasting. 
% Liu et al. \cite{LIU2020113082} proposed a recurrent neural network based dual-stage two-phase model to make long-term predictions for MTS data. 
% Lu et al. \cite{9484796} proposed a generative adversarial network combining LSTM and auto-encoder to learn representations for RUL prediction. 
% Chen et al. \cite{8998569} proposed an LSTM-based framework by combining attention to learn the importance of time steps for MTS prediction. 
% Extensive works have been devoted to leveraging sensor correlations by GNN for MTS data \cite{jin2023survey}. They mostly constructed a graph for each MTS sample and updated sensor features by leveraging sensor correlations with GNN. With the learned sensor features, they directly stacked the sensor features to learn overall representations \cite{ijcai2020-184,9280401,deng2021graph,wang2023multivariate,wu2020connecting,shao2022pre}.
% For example, Ailin and Bryan \cite{deng2021graph} captured the correlations between sensors by GNN for anomaly detection. In the last layer of GNN, they stacked all sensor features and learned the representations by a neural network.  Then, they concatenated sensor features to learn the representations for classification.
% These methods are great pioneers. However, they cannot capture the hierarchical correlations between sensors. Meanwhile, they ignored the dynamic property of MTS data. These limitations restrict their performance.
